Bayesian Persuasion with Sequential Games

We study an information-structure design problem (a.k.a. persuasion) with a single sender and multiple receivers with actions of a priori unknown types, independently drawn from action-specific marginal distributions. As in the standard Bayesian persuasion model, the sender has access to additional information regarding the action types, which she can exploit when committing to a (noisy) signaling scheme through which she sends a private signal to each receiver. The novelty of our model is in considering the case where the receivers interact in a sequential game with imperfect information, with utilities depending on the game outcome and the realized action types. After formalizing the notions of ex ante and ex interim persuasiveness (which differ in the time at which the receivers commit to following the sender's signaling scheme), we investigate the continuous optimization problem of computing a signaling scheme which maximizes the sender's expected revenue. We show that computing an optimal ex ante persuasive signaling scheme is NP-hard when there are three or more receivers. In contrast with previous hardness results for ex interim persuasion, we show that, for games with two receivers, an optimal ex ante persuasive signaling scheme can be computed in polynomial time thanks to a novel algorithm based on the ellipsoid method which we propose.

==> computing_bce.tex <==
\section{Computing Optimal \emph{Ex Interim} Persuasive Schemes}

\textcolor{red}{***citare risultato di hardness~\cite{dughmi2016algorithmic} $\#$P-hard***}

\textcolor{red}{***check On the hardness of designing public signals***}

==> extensions.tex <==
\section{Extensions}
\textcolor{red}{***heterogeneous priors and receivers with types***}

==> schemes.tex <==
\section{Persuasive Signaling Schemes}
% def BCE e BCCE
% differenze e hardness
% spigare 
% revelation principle sia per BCE che per BCCE (estendere?)
%
The usual way to characterize an \emph{optimal} signaling scheme in the multiple receivers framework is the notion of \emph{Bayes correlated equilibrium} (BCE)~\cite{bergemann2013robust,bergemann2016bayes}.
%
% persuasive scheme (IC) + perchè \Sigma
%

 
%
% revelation principle
%
%
%For players to have an incentive to follow the mediator’s recommendation in this scenario, it would have to be the case that the recommended action a i was always preferred to any other action a  i conditional on the signal t i that player i had received and his knowledge of the recommended action a i
